Do Language Embeddings Capture Scales?

Pretrained Language Models (LMs) have been shown to possess significant linguistic, common sense, and factual knowledge. One form of knowledge that has not been studied yet in this context is information about the scalar magnitudes of objects. We show that pretrained language models capture a significant amount of this information but are short of the capability required for general common-sense reasoning. We identify contextual information in pre-training and numeracy as two key factors affecting their performance and show that a simple method of canonicalizing numbers can have a significant effect on the results.

==> experiment_result_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[p]
\centering
\setlength{\tabcolsep}{2pt} %% default is 6pt
\small
\hskip-4.0cm\begin{tabularx}{\textwidth}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{Dataset} & \multirow{3}{*}{Model} & \multirow{3}{*}{Encoder} & \multicolumn{18}{c|}{Metric} \\ \cline{4-21} 
 &  &  & \multicolumn{3}{c|}{accuracy} & \multicolumn{3}{c|}{mse} & \multicolumn{3}{c|}{emd} & \multicolumn{3}{c|}{r2\_class} & \multicolumn{3}{c|}{r2\_median} \\ \cline{4-21} 
 &  &  & All & \thead{Multi- \\ modal} & \thead{Uni- \\ modal} & All & \thead{Multi- \\ modal} & \thead{Uni- \\ modal} & All & \thead{Multi- \\ modal} & \thead{Uni- \\ modal} & All & \thead{Multi- \\ modal} & \thead{Uni- \\ modal} & All & \thead{Multi- \\ modal} & \thead{Uni- \\ modal} \\ \hline
\multirow{10}{*}{\thead{All\\ Masses}} & \multirow{5}{*}{rgr} & word2vec & 0.2 & 0.19 & 0.2 & 0.088 & 0.09 & 0.086 & 0.077 & 0.076 & 0.08 & 0.29 & 0.27 & 0.34 & 0.34 & 0.32 & 0.37 \\ \cline{3-21}
 &  & BERT & 0.22 & 0.21 & 0.22 & 0.085 & 0.086 & 0.084 & 0.077 & 0.076 & 0.08 & 0.38 & 0.36 & 0.42 & 0.44 & 0.43 & 0.46 \\ \cline{3-21} 
 &  & NumBERT & 0.2 & 0.19 & 0.2 & 0.088 & 0.089 & 0.086 & 0.077 & 0.076 & 0.08 & 0.34 & 0.32 & 0.37 & 0.39 & 0.38 & 0.41 \\ \cline{3-21} 
 &  & ELMO & 0.21 & 0.2 & 0.21 & 0.087 & 0.088 & 0.085 & 0.077 & 0.076 & 0.08 & 0.38 & 0.36 & 0.41 & 0.44 & 0.42 & 0.46 \\ \cline{2-21} 
 & \multirow{5}{*}{mcc} & word2vec & 0.26 & 0.26 & 0.26 & 0.025 & 0.026 & 0.023 & 0.082 & 0.083 & 0.08 & -0.066 & -0.062 & -0.076 & -0.13 & -0.14 & -0.12 \\ \cline{3-21} 
&  & BERT & 0.33 & 0.33 & 0.33 & 0.021 & 0.022 & 0.019 & 0.062 & 0.063 & 0.06 & 0.072 & 0.055 & 0.11 & 0.097 & 0.073 & 0.14 \\ \cline{3-21} 
 &  & NumBERT & 0.32 & 0.32 & 0.33 & 0.021 & 0.022 & 0.019 & 0.057 & 0.058 & 0.055 & 0.036 & 0.015 & 0.081 & 0.068 & 0.041 & 0.12 \\ \cline{3-21} 
 &  & ELMO & 0.36 & 0.36 & 0.36 & 0.021 & 0.021 & 0.019 & 0.061 & 0.062 & 0.059 & 0.064 & 0.049 & 0.094 & 0.074 & 0.043 & 0.13 \\ \hline
\multirow{10}{*}{\thead{All\\ Lengths}} & \multirow{5}{*}{rgr} & word2vec & 0.12 & 0.12 & 0.13 & 0.099 & 0.1 & 0.097 & 0.072 & 0.07 & 0.074 & 0.19 & 0.19 & 0.21 & 0.25 & 0.24 & 0.27 \\ \cline{3-21} 
 &  & BERT & 0.24 & 0.23 & 0.24 & 0.084 & 0.085 & 0.081 & 0.072 & 0.07 & 0.074 & 0.46 & 0.45 & 0.48 & 0.5 & 0.49 & 0.51 \\ \cline{3-21} 
 &  & NumBERT & 0.22 & 0.21 & 0.22 & 0.086 & 0.088 & 0.084 & 0.072 & 0.07 & 0.074 & 0.41 & 0.4 & 0.44 & 0.45 & 0.44 & 0.46 \\ \cline{3-21} 
 &  & ELMO & 0.23 & 0.23 & 0.24 & 0.084 & 0.085 & 0.082 & 0.072 & 0.07 & 0.074 & 0.46 & 0.45 & 0.49 & 0.5 & 0.49 & 0.51 \\ \cline{2-21} 
 & \multirow{5}{*}{mcc} & word2vec & 0.3 & 0.31 & 0.28 & 0.026 & 0.022 & 0.031 & 0.079 & 0.074 & 0.087 & -0.88 & -0.85 & -0.92 & -1.03 & -1.05 & -1 \\ \cline{3-21} 
 &  & BERT & 0.42 & 0.41 & 0.42 & 0.02 & 0.021 & 0.018 & 0.056 & 0.058 & 0.054 & 0.16 & 0.14 & 0.2 & 0.12 & 0.11 & 0.15 \\ \cline{3-21} 
 &  & NumBERT & 0.4 & 0.4 & 0.41 & 0.021 & 0.022 & 0.019 & 0.052 & 0.053 & 0.049 & 0.07 & 0.056 & 0.1 & 0.032 & 0.019 & 0.059 \\ \cline{3-21} 
 &  & ELMO & 0.43 & 0.42 & 0.44 & 0.019 & 0.02 & 0.017 & 0.055 & 0.056 & 0.053 & 0.17 & 0.15 & 0.2 & 0.12 & 0.1 & 0.15 \\ \hline
\multirow{10}{*}{\thead{All\\ Prices}} & \multirow{5}{*}{rgr} & word2vec & 0.14 & 0.13 & 0.15 & 0.09 & 0.093 & 0.085 & 0.087 & 0.084 & 0.092 & 0.18 & 0.15 & 0.23 & 0.22 & 0.19 & 0.27 \\ \cline{3-21} 
 &  & BERT & 0.19 & 0.19 & 0.19 & 0.083 & 0.085 & 0.081 & 0.087 & 0.084 & 0.092 & 0.26 & 0.24 & 0.3 & 0.33 & 0.31 & 0.37 \\ \cline{3-21} 
 &  & NumBERT & 0.17 & 0.18 & 0.17 & 0.085 & 0.087 & 0.083 & 0.087 & 0.084 & 0.092 & 0.23 & 0.2 & 0.26 & 0.29 & 0.27 & 0.32 \\ \cline{3-21} 
 &  & ELMO & 0.21 & 0.21 & 0.22 & 0.081 & 0.083 & 0.078 & 0.087 & 0.084 & 0.092 & 0.33 & 0.3 & 0.37 & 0.4 & 0.38 & 0.44 \\ \cline{2-21} 
 & \multirow{5}{*}{mcc} & word2vec & 0.26 & 0.25 & 0.28 & 0.019 & 0.014 & 0.024 & 0.063 & 0.055 & 0.072 & -0.65 & -0.71 & -0.58 & -0.83 & -0.97 & -0.7 \\ \cline{3-21} 
 &  & BERT & 0.33 & 0.32 & 0.33 & 0.017 & 0.019 & 0.014 & 0.054 & 0.055 & 0.051 & -0.24 & -0.27 & -0.18 & -0.3 & -0.35 & -0.24 \\ \cline{3-21} 
 &  & NumBERT & 0.32 & 0.32 & 0.33 & 0.017 & 0.019 & 0.014 & 0.051 & 0.053 & 0.048 & -0.35 & -0.4 & -0.26 & -0.44 & -0.5 & -0.34 \\ \cline{3-21} 
 &  & ELMO & 0.37 & 0.36 & 0.38 & 0.016 & 0.018 & 0.013 & 0.051 & 0.053 & 0.047 & -0.098 & -0.14 & -0.036 & -0.15 & -0.21 & -0.074 \\ \hline
\multirow{10}{*}{\thead{Animals\\ Masses}} & \multirow{5}{*}{rgr} & word2vec & 0.35 & 0.35 & 0.36 & 0.069 & 0.069 & 0.069 & 0.077 & 0.081 & 0.07 & 0.35 & 0.39 & 0.26 & 0.38 & 0.43 & 0.29 \\ \cline{3-21} 
 &  & BERT & 0.26 & 0.26 & 0.24 & 0.079 & 0.076 & 0.085 & 0.077 & 0.081 & 0.07 & 0.13 & 0.12 & 0.13 & 0.15 & 0.13 & 0.18 \\ \cline{3-21} 
 &  & NumBERT & 0.23 & 0.23 & 0.24 & 0.083 & 0.081 & 0.086 & 0.077 & 0.081 & 0.07 & -0.026 & 0.05 & -0.17 & -0.0092 & 0.055 & -0.1 \\ \cline{3-21} 
 &  & ELMO & 0.28 & 0.25 & 0.33 & 0.079 & 0.08 & 0.077 & 0.077 & 0.081 & 0.07 & 0.17 & 0.17 & 0.17 & 0.19 & 0.21 & 0.16 \\ \cline{2-21} 
 & \multirow{5}{*}{mcc} & word2vec & 0.33 & 0.32 & 0.35 & 0.021 & 0.02 & 0.023 & 0.069 & 0.066 & 0.075 & 0.062 & 0.06 & 0.064 & 0.059 & 0.065 & 0.05 \\ \cline{3-21} 
 &  & BERT & 0.41 & 0.39 & 0.45 & 0.017 & 0.016 & 0.019 & 0.058 & 0.057 & 0.06 & 0.13 & 0.063 & 0.24 & 0.16 & 0.11 & 0.25 \\ \cline{3-21} 
 &  & NumBERT & 0.42 & 0.43 & 0.41 & 0.018 & 0.016 & 0.02 & 0.053 & 0.052 & 0.055 & -0.0071 & 0.075 & -0.16 & -0.11 & -0.00052 & -0.26 \\ \cline{3-21} 
 &  & ELMO & 0.43 & 0.44 & 0.42 & 0.016 & 0.015 & 0.019 & 0.057 & 0.056 & 0.059 & 0.2 & 0.24 & 0.14 & 0.17 & 0.22 & 0.095 \\ \hline
\multirow{10}{*}{\thead{Household\\Product\\ Prices}} & \multirow{5}{*}{rgr} & word2vec & 0.45 & 0.43 & 0.48 & 0.056 & 0.058 & 0.055 & 0.092 & 0.094 & 0.09 & 0.12 & 0.15 & 0.037 & 0.27 & 0.31 & 0.2 \\ \cline{3-21} 
 &  & BERT & 0.44 & 0.42 & 0.46 & 0.057 & 0.059 & 0.055 & 0.092 & 0.094 & 0.09 & 0.12 & 0.15 & 0.057 & 0.24 & 0.26 & 0.2 \\ \cline{3-21} 
 &  & NumBERT & 0.42 & 0.39 & 0.46 & 0.06 & 0.062 & 0.057 & 0.092 & 0.094 & 0.09 & 0.055 & 0.077 & -0.0021 & 0.16 & 0.2 & 0.086 \\ \cline{3-21} 
 &  & ELMO & 0.42 & 0.4 & 0.46 & 0.058 & 0.059 & 0.057 & 0.092 & 0.094 & 0.09 & 0.089 & 0.12 & 0.018 & 0.24 & 0.29 & 0.13 \\ \cline{2-21} 
 & \multirow{5}{*}{mcc} & word2vec & 0.51 & 0.49 & 0.54 & 0.0083 & 0.0084 & 0.0081 & 0.041 & 0.041 & 0.041 & 0.02 & 0.0099 & 0.028 & -0.001 & -0.025 & 0.028 \\ \cline{3-21} 
 &  & BERT & 0.57 & 0.56 & 0.58 & 0.0072 & 0.0073 & 0.007 & 0.038 & 0.038 & 0.039 & -0.039 & -0.054 & -0.021 & -0.18 & -0.22 & -0.14 \\ \cline{3-21} 
 &  & NumBERT & 0.55 & 0.53 & 0.57 & 0.0075 & 0.0075 & 0.0075 & 0.038 & 0.038 & 0.039 & -0.061 & -0.055 & -0.087 & -0.21 & -0.2 & -0.24 \\ \cline{3-21} 
 &  & ELMO & 0.54 & 0.52 & 0.57 & 0.0073 & 0.0073 & 0.0073 & 0.038 & 0.038 & 0.039 & -0.033 & -0.047 & -0.017 & -0.16 & -0.19 & -0.14 \\ \hline
\end{tabularx}
\caption{Experiment results}
\label{tab:all_results}
\end{table*}
